ViCA-NeRF: View-Consistency-Aware 3D Editing of Neural Radiance Fields

We introduce ViCA-NeRF, the first view-consistency-aware method for 3D editing with text instructions. In addition to the implicit neural radiance field (NeRF) modeling, our key insight is to exploit two sources of regularization that explicitly propagate the editing information across different views, thus ensuring multi-view consistency. For geometric regularization, we leverage the depth information derived from NeRF to establish image correspondences between different views. For learned regularization, we align the latent codes in the 2D diffusion model between edited and unedited images, enabling us to edit key views and propagate the update throughout the entire scene. Incorporating these two strategies, our ViCA-NeRF operates in two stages. In the initial stage, we blend edits from different views to create a preliminary 3D edit. This is followed by a second stage of NeRF training, dedicated to further refining the scene's appearance. Experimental results demonstrate that ViCA-NeRF provides more flexible, efficient (3 times faster) editing with higher levels of consistency and details, compared with the state of the art. Our code is publicly available.

==> Figure/geo.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Figure/geometry.pdf}
    \captionsetup{type=figure}
\vspace{-8mm}
    \captionof{figure}{\textbf{Edit Contextual Elements:} Though using depth-guided correspondence, our method is also able to operate on contextual elements that can modify content.}
    \vspace{-5mm}
    \label{fig:geo}
\end{figure}

==> sup_figure/prompt.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c|c|c}
\toprule
Method & Text-Image Direction Score & Temporal Consistency Score\\ \hline
Instruct-NeRF2NeRF         & 0.1016 & 0.5161   \\ 
ViCA-NeRF (Ours)                  & \textbf{0.1412} &\textbf{0.6498}   \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Quantitative evaluation on difficult edits.}Evaluated on 10 edits on scenes from Instruct-NeRF2NeRF~\cite{in2n}. Our method performs better on both metrics.}
\vspace{-5pt}
\label{tab:hard}
\end{table}
